Tapping the sensorimotor trajectory

In this paper, we propose the concept of sensorimotor tappings, a new graphical technique that explicitly represents relations between the time steps of an agent's sensorimotor loop and a single training step of an adaptive internal model. In the simplest case this is a relation linking two time steps. In realistic cases these relations can extend over several time steps and over different sensory channels. The aim is to capture the footprint of information intake relative to the agent's current time step. We argue that this view allows us to make prior considerations explicit and then use them in implementations without modification once they are established. Here we explain the basic idea, provide example tappings for standard configurations used in developmental models, and show how tappings can be applied to problems in related fields.

==> tappingsbody_arxiv_v1.tex <==
\section{Introduction}
\label{sec:orge25b6d6}

% \FIXMET{Clean out math details from intro}

%% drix: No hard rule again but some heavy sentences could be made to
%% flow better in the active tense.

%% drix: many sentences say two separate things and could advantageously
%% be split.

%% drix: complex phrase

%% drix: verbs vs. nouns

%% drix: A B vs. B of A, internal model accuracy vs the accuracy of
%% internal models

%% drix: definite articles: the

%% general: kill acronyms

% \FIXMET{Introduce example in intro}

%% general: disambiguate the two modelling levels by calling the inner
%% supervised learner ``sensorimotor model'' and the developmental model
%% ``developmental model''.

% bib clean up
% \cite{sutton16:introrl} -> \cite{Sutton98}

\myparb{Agent development} Looking at developmental processes in
higher animals reveals that they involve large amounts of learning
from experience. Developmental Robotics, in agreement with Reinforcement
Learning and Computational Neuroscience, is concerned with evaluating
hypothetical principles of development and learning. Although the fields differ in
motivation, evaluation happens to a large extent through computational
models in which the principles are represented as patterns of
interaction between a number of adaptive components with specific
functions.

%% Most theories of the development of higher animals and artifical
%% agents agree, that a large amount of data driven learning is involved
%% at all times. The fields of Developmental Robotics, Reinforcement
%% Learning and Computational Neuroscience all contribute detailed
%% theories about the organization of these learning processes and their
%% objectives. There is less agreement regarding the details, and this
%% results in a large number of proposals that are sometimes 
%% hard to disentangle or to compare on equal grounds.

%%  physical processes that
%% interaction with
%% the environment. 

\myparb{Learning as modelling} A generally accepted view
is that the agent's brain contains modules which function as models of
the agent's interaction with the world. The idea is that these
models are used by the brain to evaluate the possible actions in
``imagined space'' and only commit to the most promising one in
physical space. The task of a theory now is to describe precisely how
a sensorimotor model is learnt from experience and how it interacts
with other models present within the context of a developmental model.

\myparb{Levels of modelling} We need to emphasize this distinction
between different types of models. Machine learning (ML) solves the
problem of how to build models from data in a problem independent
form. The ML approach relies on a \emph{preprocessing step} to
transform the raw data into the required form. Using ML methods we can
learn sensorimotor models of transitions in sensorimotor space up to a 
desired accuracy. This
level of modelling provides the grounding in sensorimotor
space. Developmental models need to capture the preprocessing and
the interaction of the sensorimotor models that they
contain. Sensorimotor models can have different roles which are
determined by the relations contained in the training data. An
important question is \emph{how to map the raw sensorimotor data to
  sensorimotor training data} for realizing specific functions needed
inside a developmental model.

\begin{figure}
  \centering
  % \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width=0.4\textwidth]{img/p_tappings/ex_tpg_nao_1.pdf}
    \caption{Example: On the left a Nao robot trains a model to predict visual consequences from
      joint angle configurations through sensorimotor exploration,
      right: the robot uses the model to find the best matching
      prediction and the associated action in the predictor's input.}
    \label{fig:ex-1-nao-hand-three}
  %\end{subfigure}
\end{figure}


\myparb{Example} Consider a simple example from robotics involving an
experiment like the one shown in \autoref{fig:ex-1-nao-hand-three}. A
humanoid robot is bootstrapping the ability to move one of its hands
to a specified point in the visual space of the robot's camera. For
simplicity the camera does not move. The robot's arm has four joints
and the hand's position is determined by the configuration of all four
individual joints taken together. The agent records a series of random
joint angle commands and corresponding camera images. Using these
data, it trains a sensorimotor model to predict the resulting camera
image from the joint angles that generated it. Finally the agent
exploits the trained model by feeding random commands into the model,
recording the predictions and choosing the commands which result in
the prediction closest to the goal. For all of this to work, the
sensorimotor training data at any time step need to be composed of the
image at that same time step and the command from the previous time
step. In the rest of the paper we develop a graphical technique for
representing and analzying such mappings from sensorimotor time steps to training steps.


%% Functionally the l1-models
%% perform prediction and inference in sensorimotor space while the
%% l2-models generate behavior on the basis of the l1-models activity.

%% These models are fundamentally grounded
%% in sensorimotor data but have limited scope. 

%% The \emph{learning} consists of creating models that capture
%% regularities in the experience data.

%% \subsection{Model basics and terminology}
%% \label{sec:model_basics_and_terminology}

% Distinguish models at ML level and models at dev level.

%% and with 
%% error-based methods

%% , unlocking the toolbox of (supervised) Machine
%% Learning.

%% \FIXMET{make $S_E$ blocks with little images inside to
%%       indicate vision}

\begin{figure*} % [htb!]
  \centering
  % \includegraphics[width=0.96\textwidth]{img/p_tappings/smt_tapping_basic.pdf}
  % \includegraphics[width=0.96\textwidth]{img/p_tappings/smt_tapping_improved.pdf}
  \includegraphics[width=0.96\textwidth]{img/p_tappings/smt_tapping_improved_reversed.pdf}
  \caption{\label{fig:basic-idea} The basic idea of tapping the
    sensorimotor trajectory. Concatenating the row vectors horizontally
      creates a matrix. The matrix inherits the row structure from the
      vector and represents time along the other axis.}
  %% \caption{\label{fig:basic-idea}\textbf{Tapping:} the basic idea. The
  %% cloud on the right is the sensorimotor space. The black circle represents
  %% the agent's current position in that space. At every time $t$
  %% we sample one such point, producing the vector $\bm{sm}_{t}$. Each
  %% vector is attached to the growing matrix $\bm{SM}$ from the
  %% right. If the episode is finite the matrix will be finite too, if
  %% the episode is infinite, we still need to consider a finite scope of
  %% information intake.}
  % \FIXMET{change row colors of m and $s_e$}
\end{figure*}

\subsection{Related work}
\label{sec:org8f62a06}

% \FIXMET{Describe the related work and show that time+interaction are not covered}

%% By leaving out details, any of these descriptions can become
%% ambiguous with respect to the precision required for an algorithmic
%% description.

\myparb{Modelling tools} The techniques most commonly used for
discussing developmental models are either plain textual descriptions,
equations in formal approaches, or variations of block diagrams
and signal-flow diagrams on the graphical side. Nothing in general can be
said about plain text descriptions. Equations and flow diagrams are
usually highlighting different but fixed aspects of the model's
function or the design problem. Equations are precise in
representing functional dependencies and time. Block- and flow
diagrams tend to emphasize the structure of interaction among the
variables of interest. For analysis, these techniques are usually
complemented by problem specific graphical representations of
behaviour.

%%  which
%% preserves the relational precision of 
%% equations and the graphical accessibility of diagrams.

%% In the rest of
%% the paper we will introduce the idea in more detail, illustrate it by
%% means of an example and discuss tappings for prototypical models often
%% used in the field.

%% The body of work on developmental learning is huge and due to the
%% field's interdisciplinary nature many different frameworks exists
%% within which models are designed, analyzed and discussed. Established
%% ones are mathematical
%% modelling with equations, and graphical modelling with signal flow,
%% block or freestyle diagrams. Any framework usually has to trade-off
%% the level of block abstraction with the explicitness of block
%% function. Like.

% needs rewrite:



% \FIXMET{Rewrite} \textbf{Related work:}
The visualisation and conceptualisation techniques are coming largely
from electrical diagrams, signal processing and control theory. The
ideas of black boxes and modular design, as they are used in block
diagrams, is rooted in these fields as well. The black box view allows
for general input/ouput analyses. The corresponding equations, for
example discrete state space based iterative update rules, equally
reflect their origin in the formalisms of these areas. A notable
exception are the backup diagrams introduced by Sutton \& Barto in
\cite{Sutton98}. Backup diagrams track how the instantaneous
information is related to previous states and indicates how it is
propagated back in time to update the relevant state in the agent's
controller. These diagrams do not however differentiate sensory
modalities.

%% This principle, free energy minimization
%% through prediction,

%% provides the connection from the neural
%% perspective to other models


% start with a concrete example!
\myparb{Signal processing} The most important concept in digital
signal processing for time domain manipulation is the finite impulse
response filter. Such a filter's output is computed as a weighted sum
over a finite number of past inputs including the current one. It is
realized by \emph{tapping} into a sliding window over inputs with
fixed real-valued weights. Each weight corresponds to a fixed delay
and the largest delay with a non-zero weight is the maximum time
across which there can be causal interaction between input and output.

%% A
%% filter equation specifies real valued coefficients for 
%% tapping two different delay lines, one for input values and one for
%% filter outputs (global feedback memory).

%%  are literally pure
%% tappings.

%% The tools described so far take an inside
%% view of what constitutes a developmental model.

%% bib clean: dersteinpas99, 2010arXiv1004.2515W

\myparb{Information theory} Information theory can be applied to
analyze the information flow across the inputs and outputs of a black
box to characterize general properties of information \emph{shared}
among these variables. Information theoretic analysis of sensorimotor
relations can be made quantitative \cite{Lungarella2005} and has been
proposed as a way to capture high level properties of experience
\cite{Tononi24051994}. A number of recent proposals for modelling
behaviour as a self-organizing process have suggested to measure
information sharing over time \cite{1999cond.mat..2341B} and to use
that measure for driving behaviour
\cite{der2012playful,PMID:23723979,10.1371/journal.pone.0004018}. This
can be taken as evidence for the importance of predictability for
guiding agent-environment interaction. The dependence of
predictability on the amount of past experience going into the prediction
allows to precisely determine the memory needs of a given agent.

%%  the long-term behaviour of the
%% prediction error naturally

%%  It 
%% turns out that a common measure in these proposals involves the
%% statistics of the moment-to-moment prediction error.

% charts. Input/Output diagrams/analysis, black-boxing,

% \FIXMET{signal processing comes here or later in the implementation section}

% auto-regression, Bayes filtering
% including auto-association, and conditional inference.


\myparb{Contribution} Internal modelling approaches in
developmental robotics that use prediction learning are missing a way
to describe in a general and systematic manner the interaction of the
embedded sensorimotor models with the information provided by the enclosing
developmental model. This also holds for temporal difference learning
in RL and correlational learning processes in neuroscience. Thus we
see a definite need for an additional tool from which these fields,
and maybe robotics and AI at large, might benefit. Our contribution 
besides the identification of this gap is a proposal for filling it.

% \FIXMET{Hebb, R-W, Niv, Dayan, Wörgötter, Clark, Friston, Predictive Brain}.
%% From the relevant literature we extract an apparent invariant across
%% many approaches:the central presence of
%\myparb{Invariant} \FIXMET{



%% That tool
%% should allow us to make more efficient use of pervasive concepts such
%% as \emph{temporal difference learning}, \emph{prediction learning},
%% and the \emph{sensorimotor loop}.

%% We argue that the SML view emphasizes the single
%% timestep information flow over situations that are more spread out. If
%% we superimpose the minimal temporal relation as a graph on the matrix
%% grid and extend it inside the grid space, we can capture non-temporal
%% prediction scenarios, for example \emph{Associative learning}.


% with various configurations of conditional mutual information
%% \FIXMET{Der, Martius, Ay,
%%   Zahedi, Polani, Salge, Friston}.

%% Finally, the method of partial information decomposition \FIXMET{ref} aims to
%% achieve related quantifcations of strength, type and distribution
%% variable interdependence. And Lungarella, Sporns et al.

\section{Tappings}
\label{sec:model_basics}

%% Learning agents thus require innate
%% search and exploration behaviours to be able to start the
%% bootstrapping process

%%  whose elements each contain
%% an instantaneous measurement from one single receptor.

% , motors, and state variables

%% During its
%% lifetime the agent samples the sensorimotor space and creates a new
%% measurement vector at every time step.

% Take a look at . It is meant to complement this section and

\myparb{Sensorimotor space} The sequence of steps necessary for going
from sensorimotor space to the sensorimotor models's input / output
space are shown in the illustration in \autoref{fig:basic-idea} with a
blow-up of the tapping transformation. In order to learn, an agent
must produce information through actions that produce changes in the
outside world. The information becomes available to the agent
\emph{exclusively} through its sensors \footnote{To simplify the
  discussion, we use \emph{sensors} as a placeholder for any kind of
  internal state variable. These are either primary signals, like the
  actual sensors, motors or basic rewards, but also signals derived
  from any intermediate stage in the agent brain's flow of
  computation.}. A single sensory measurement is usually represented
by a vector. The vector is composed of subparts that reflect the
natural structure given by the types of the sensors, which correspond
to \emph{modalities} (e.g. vision or joint angles). The set of all
possible vectors defines the agent's sensorimotor space. The agent's
internal time creates the temporal ordering of incoming measurements
\cite{10.3389/frobt.2016.00004}, and storing them in this order forms
a matrix. The matrix contains a numerical representation of the
sequence of changes in the real world \emph{as they are reflected} in
sensorimotor space. If the agent lives in a world that is not
completely observable (pretty much every world), it must squeeze out
additional information by exploiting relations across time and across
modalities. To do this it must tap the sensorimotor matrix using a
fixed pattern attached to the current time step with the growing
matrix sliding along underneath.

\begin{figure}
  \centering
  % \begin{subfigure}[b]{0.45\textwidth}
  \includegraphics[width=0.4\textwidth]{img/p_tappings/ex_tpg_nao_2.pdf}
    \caption{Example cont.: This illustrates the remapping of time
      that the Nao agent needs to realize when constructing the
      training data, input $\bm{X}$ and labels $\bm{Y}$, from the raw
      sensorimotor data in this particular example.}
    \label{fig:ex-2-nao-remapping}
  %\end{subfigure}
\end{figure}

\myparb{Example} Before examing this in more detail let's see how this
translates back into our example. A humanoid robot is bootstrapping
the ability to move its hand to a given point in visual space. The
agent creates information by generating random joint angle commands
and recording the resulting image. For simplicity we say that the
motion of the arm is finished by the time the next image is
taken. Each measurement vector contains the \emph{current} image, the
previous command's consequence, and a \emph{new} motor command about
to be committed \footnote{This ordering is only a convention but in
  our view the most intuitive one.}. The agent records measurements
over 5 time steps and trains an internal forward model to predict the
image in the current time step from the previous time step's joint
angle command. To do this, the agent constructs a training set for an
adaptive model. The textual description is complicated although the
relation is very simple as shown in
\autoref{fig:ex-2-nao-remapping}. The agent aligns the motor commands
from the first to the second to last values as the input, and the
images from the second to the last image as the target to construct a
matrix of 5-1 training data points. The relation in this example is
trivial but already contains the essential ingredients connecting two
different modalties across two time steps. The prediction happens
within one time step but its input can extend over any number of time
steps.

%% The agent's sensorimotor loop discretises time and
%% thereby creates a new vector at every step.

 %% tied to the time
 %% experienced by the agent
 
%% It can also be
%% seen as the unrolled agent states over discrete time

% time dimension.

%% and capture the activity of
%% the agent over time and the motion of the 

%% A set of
%% data points arranged in this order 

% is a sensorimotor trajectory%%  which can be captured and
%% represented in a matrix SMT by concatenating single measurement
%% vectors along the time axis.

%% comprising all points in sensorimotor space that can in
%% principle be visited by the agent. 
%% correspondences 

%% A single sample can be represented by a vector that contains the instantaneous values of all agent-internal
%% observables.

%% resulting in a new vector
%% creating 

%% of elements with observable types such sensors, rewards, motor
%% commands or higher-level internal states computed from primary
%% sources.

% \FIXMET{cite space paper: Terekhov AV and O'Regan JK (2016) Space as
% an Invention of Active Agents. Front. Robot. AI 3:4. doi:
% 10.3389/frobt.2016.00004}

%%   in a minimal sense is
%% to reduce $n$ bits of particular information to $k < n$ bits of more
%% general information.


%% \myparb{From SMT to XY} Low-level theories of learning have to be precise about
%% \emph{what} is adapted based on \emph{which} piece of information. The
%% precise routing and assignment of variables, the elements of the
%% matrix $\bm{SMT}$, to inputs $\bm{X}$ and targets $\bm{Y}$ of
%% trainable function approximators is an important and error-prone task
%% in computational modelling (CM) of developmental processes.

%% \FIXMET{marginpar: Anticipation vs. prediction} Many computational theories of
%% development and learning rely on the idea of anticipation
%% (\cite{rosen12:anticipatory_systems}). Technically, anticipation in
%% behaviour will be realized with predictive models of some sort. These are generally
%% conceived of as adaptive models that learn individual statistics. By
%% virtue of prediction learning they can be trained with fast supervised
%% learning rules.


% \section{Tapping}
% \label{sec:org81add03}
% (\autoref{sec:org81add03}

\myparb{From sm-space to sm-matrix.} Now we are prepared for a
detailed account of the tapping procedure. Models of interacting
agents usually have a fixed number $n_s$ of sensors and a fixed number
$n_m$ of motors, both represented as column vectors. Each vector has
additional internal structure reflecting different types and groups of
sensors and actuators. In \autoref{fig:basic-idea} for example we are
using four different modalities: motors, proprioception, exteroception
and interoception, denoted by $\bm{M}$, $\bm{S}_{\text{P}}$,
$\bm{S}_{\text{E}}$ and $\bm{S}_{\text{I}}$ respectively. To obtain a
general representation we concatenate all these vectors into one large
column vector $\bm{sm} \in \mathbb{R}^{n_{sm}}$ with dimension
$n_{sm}$ holding all sensorimotor variables. All possible realizations
of $\bm{sm}$ span the sensorimotor space $\bm{SM} =\mathbb{R}^{n_{sm}}$. In
most cases the agent cannot actually realize all physical
correspondences with points in $\bm{SM}$. The set of actually reachable states is
called the sensorimotor manifold. The sensorimotor loop adds a
discrete time $t$ for every iteration it is going through. For every
$t$ there is a realization $\bm{sm}_t$ of the sensorimotor vector. We
collect all of these and store them side by side in the sensorimotor
matrix $\bm{SMT}$.


%%  for every episode of agent
%% activity. 

%% For every episode of agent
%% activity there is one such matrix that contains the state trajectory
%% of that episode. Alternatively, $\bm{SMT}$ , much like a recurrent neural network is
%% unrolled before applying backpropagation.

%% Assuming a fixed sampling rate (the execution rate of the
%% sensorimotor loop) there is one such vector for every timestep \(t\)
%% denoted \(sm_t\). These can be concatenated over all \(t\) creating
%% the matrix SM which then holds the temporally unrolled sensorimotor
%% loop, representing a trajectory. This sequence of steps is shown in
%% \autoref{fig:basic-idea}.

%% All the vectors
%% attached to a specific sensor can be concatenated into one large
%% sensor vector \(s\) and the same can be done with all actuator vectors
%% to obtain a larger motor vector \(m\). \(s\) and \(m\) in turn can be
%% joined into a single sensorimotor vector \(sm\). 

%% \myparb{SM to SMT} We now want to give a detailed account of the
%% tapping procedure. Subvectors $s_p$, $s_e$, $s_m$. Cat onto sm. Space
%% spanned by by sm is SM. Matrix of sm vectors over time is SMT.

% that the loop is going through

%% Different computational models of developmental learning mostly differ
%% in two ways. One specifies how the model interfaces with the outside,
%% specified by which variables are predicted on the basis of which other
%% variables and at which times, the other is the mechanics of how the
%% prediction is computed and adapted.

A common arrangement in a developmental model is to use a single
learning algorithm inside a box for representing an internal
model. Such a model is most effectively trained with supervised
learning. A supervised training set consists of input data $\bm{X}$
and target data $\bm{Y}$ that constrain the functional relation
$f(\bm{X}) = \bm{Y}$. The approximation task is to find parameters
$\theta$ for the model $\hat f(\cdot, \theta)$ such that $|f - \hat
f|$ is minimized under some measure. Prediction learning allows the
agent to construct infinite supervised training data on the fly. What
is missing is a systematic way to describe that construction process.

% and  method because we used the tapping to create a supervised training
% set.

To fill this gap we propose \textbf{tappings} and define them as
directed graphs on top of $\bm{SMT}$'s row and column coordinates. Each
node of the graph is placed on a cell of the matrix and assigned an
input or target color. The tapping is defined relative to the current
time $t$ with the data sliding along under the tapping 
with each time step. If $\bm{XY}$ is the full supervised 
training set, the tapping defines a map taking a set of
$\bm{SMT}$ coordinates to a set of $\bm{XY}$ coordinates. The node
coordinates on the $\bm{SMT}$ grid encode the relation prescribed by
the sensorimotor model's function inside the developmental model.

%% The tapping is usually locally confined with respect to time \(t\) of SMT. Setting one
%% cell as the origin, the positions of all other markers can be given
%% relative to that. This anchorpoint can now be shifted along \(t\)
%% producing a data point for every step \(t\) of SML containing a subset of
%% the values of SMT cells selected according to a well-defined
%% spatiotemporal relation.



%% \footnote{A map linking a
%%   vector of grid positions to another vector of grid 
%% positions. Taking the n-fold cross-product of the space of grid
%% positions to the m-fold cross-product of the space of grid positions.}. The
%% markers are labelled with the inputs and outputs of the elements in
%% the model of interest.

%% \[ GP^n \mapsto GP^m \]

\begin{figure}
  \centering
  %% \begin{subfigure}[b]{0.45\textwidth}
  %%   \includegraphics[width=0.1\textwidth]{img/p_tappings/ex_tpg_nao_3.pdf}
  %% \end{subfigure}
  %% \vspace{2pt}
  \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{img/p_tappings/ex_tpg_nao_3b.pdf}
  \end{subfigure}
  \caption{Tapping for the nao example with a corresponding block diagram.}
  \label{fig:ex-3-nao-tapping}
\end{figure}

\myparb{Example} Returning to our example one more time we can now
write it down as the tapping shown in
\autoref{fig:ex-3-nao-tapping}. The Nao agent's sensorimotor space consists
of four motor values and an image. For simplicity we leave away the
details of image processing. During exploration the agent creates a
sensorimotor trajectory from which it learns to predict
visual consequences from joint angle commands. By design of the experiment
there is a delay of one time step between committing a motor
command and measuring the results associated with that command. This
means that every time there is a new image measurement the agent
creates a new training data point by concatenating the current image
with the previous command and performs a single update step on the
internal model.

% \FIXMET{missing example / picture}


%% In this specific context, the tapping provides a precise and
%% explicit prescription of how the supervised dataset for a function
%% approximator (FA) can be constructed from SMT, illustrated in
%% \autoref{fig:basic-idea}. In an extended context, more complicated
%% situations involving more than one \FIXMET{model components} can be
%% formulated as a tapping, for analysis and comparison but here we only
%% look at the simple case of one FA.



%% From our point of view tappings enrich the DevRob modelling toolkit with
%% the following key items:

%% \emph{information hull}\footnote{Surprise: info hull is the joint
%%   entropy. As in e.g. convex hull.}  (e.g. the mutual information
%% between X and Y) providing a reference for comparison of information
%% efficiency.

%% \subsection{Structure of the matrix}
%% \label{sec:orge847b5c}

\subsection{Tapping degrees of freedom}
\label{sec:org0564aaf}


% \FIXMET{sentence to complex}
The design space of tappings established it needs to be examined for
the possibilities of systematic variation. \myparb{Row structure} The
variables used for a given agent are commonly grouped during the
definition of $\bm{sm}$ according to a few main properties of the what
the variable represents. They are distinguished according to wether
the variable encodes a sensor or motor signal, and then again
according to lower level properties such as exteroceptive- (vision,
hearing), proprioceptive- (joint angles, forces), or
\emph{interoceptive} signals. Interoceptive variables represent any
intermediate stage of the computations in the agent's sensorimotor
integration process. The term is based on the idea that the brain can
deploy sensor probes to any location inside the circuits that define
its own operation. Blocks of different color in a tapping indicate the
group. A group  whose elements all contribute to the same argument of
the desired function, for example all pixels in an image, it can be
reduced to a single element in the graphical representation. Groups
are organized along the row axis of the matrix representing modalities.

%% Variables be grouped by their location on the body
%% or by the type of physical effect that they produce.

%% In
%% these cases the labelling implies that the information is distributed
%% among all elements of the vector.

\myparb{Column structure} Tappings are specified relative to the
current time $t = 0$, becoming positive in the future and negative
into the past. This proposal only considers discrete time and
equidistant sampling with a constant \(\Delta t\). The sampling
interval needs to be tuned to match the processes the agent needs to
observe and to provide sufficient time to compute one iteration of the
sensorimotor loop. Loop iterations are unrolled along the column axis
of the matrix representing agent time.

%% which can also be seen as the unrolled sensorimotor
%% loop.

% \begin{wrapfigure}{l}{0.5\textwidth}% [htb!]
\begin{figure}% [htb!]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{img/p_tappings/ex_tpg_simplepred.pdf}
    \caption{Simple temporal predictor.}
    \label{fig:ex-tpg-simplepred}
  \end{subfigure}
  \vspace{2pt}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{img/p_tappings/ex_tpg_intermodal.pdf}
    \caption{Simple intermodal predictor.}
    \label{fig:ex-tpg-intermodal}
  \end{subfigure}
  \caption{The two principal axes of association shown as tappings
    alongside with corresponding block diagrams. a) A simple temporal
    predictor, predicting the state one timestep ahead, and b) a
    simple intermodal predictor taking proprioceptive input to a
    exteroceptive prediction.}
\end{figure}

% Taking a slightly broader view, 
%%   are across the time axis (matrix
%% columns) and the modalities (matrix rows).

\myparb{Time} These are the principal axes of association along which
a model can learn a functional relation. A single time step prediction
problem requires a tapping which assigns a variable at \(t-1\) to the
input and the same variable at time \(t\) to the target of a model
update. \myparb{Modality} Doing the same along modalities captures
intermodal prediction, that is, predicting sensory consequences in one
modality from the state of another modality. Adding joint angle
sensors the Nao agent it could learn to predict the hand position
(vision) from joint angles (proprioception) in the same time
step. These two proto-tappings from which all others can be composed
are shown in \autoref{fig:ex-tpg-simplepred} and
\autoref{fig:ex-tpg-intermodal}.

 %% \footnote{Presented with
 %%  three pictures of the same object in different colors we don't
 %%  explain that by reciting the luminance values of the image pixels
 %%  but by saying cat, in red, green and yellow.}

%% A fundamental objective of \emph{learning} is
%% generalization. It enables the learner to explain a large number of
%% observations with a smaller number of explanatory causes. 

%% For an interacting agent, an important part of
%% developmental learning is to approximate rules that explain regularity
%% in sensorimotor state transitions in time and modality.

%% The forward model predicts consequences at the output
%% based on causes provided as the input.

%% Take as an example an agent's
%% ability to predict the reappearance of a moving object passing behind
%% another object that is blocking the view. From the motion parameters
%% that the agent measured before the object disappears it can predict
%% the position for the next few moments, in particular the moment of
%% reappearance.

%% Such rules of change can be analytically modelled with
%% differential equations which can be turned into simulations.

Sensorimotor models encode regularity in sensorimotor state
transitions along these axes. \myparb{Forward change} Learning
transitions along the normal forward flow of time results in a forward
model. Forward models are central to the simulation theory of
cognition. The theory states that an agent learning to approximate the
forward transition rules to a sufficient degree of fidelity can use
them to interally ``simulate experience'' \cite{Hesslow201271}.

%% The fidelity of such simulations depends
%% crucially on the accuracy of the learnt model as small errors 
%% accumulate over 

%% In terms of the sensorimotor data matrix this means predicting the
%% values at some matrix elements based on the input from some other
%% elements. This view immediatly suggests prediction backwards in time.
% DONE: Hesslow G. (2012), The current status of the simulation theory
% of cognition. Brain Res.1428:71-9.


%% from its experience
%% is to learn the lawfulness inherent

%% allowing relations among different parts of the full state vector to
%% also count as transitions.


%% This can be seen as learning a partial
%% differential equation (PDE) of the system specified by the agent's
%% internal variables and their interaction, the lawful change of state
%% across time or modality expressed using earlier states and their
%% derivatives. The PDE, approximated by an internal model inside the
%% agent's brain, can be used to predict the likelihood of future
%% states. 

%%  Making the direction of the sensorimotor
%% model's prediction point backwards in time

%% reverses time and

%% prediction can go backwards in time inverting the forward change.

\myparb{Backward change} Rearranging the direction of prediction to go
backwards in time using the same set of variables used in the forward
model. This allows the model to predict (infer) causes from observed
effects. Technical details aside, this allows an agent to control and 
change its own state by directly predicting the causes of its desired
state. This translates to predicting the actions that lead to a goal
\cite{Rolf:2015}. This is a functional capability which can be
implemented by sampling forward simulations or as a single prediction
step. Direct prediction has a technical requirement on the learning
algorithm. The inverse of a function is not garantueed to be a
function itself but instead relate a single consequence to multiple 
causes. The mathematical object is called a correspondence and the
problem can be solved with learning algorithms using probabilistic
representations.

%% This means that we can safely disregard these underlying
%% issues when consdering tappings. Interestingly an inverse model can be
%% implemented by black-boxing a search over multiple forward simulation
%% outcomes.


%% that are predicted as causes of
%% a goal state, enabling goal directed behaviour. In other words, if the
%% agent is able to predict a cause (action) from an effect (desired
%% state) it can reliably reproduce that effect whenever needed, which
%% amounts to reaching the goal . 

%% There are technical
%% issues that need to be considered though. So far we have only talked
%% about function approximation. The inverse of a function might not
%% be a function itself but instead relate one consequence to multiple
%% causes. Such an object is called a correspondence and the problem can
%% be solved by using probabilistic representations in sensorimotor
%% models. This means that we can safely disregard these underlying
%% issues when consdering tappings. Interestingly an inverse model can be
%% implemented by black-boxing a search over multiple forward simulation
%% outcomes.

%% (a function is forbidden to map one input on more than one
%% outputs).
% DONE: Rolf, M., and M. Asada, "What are goals? And if so, how
% many?", IEEE Int. Conf. Development and Learning and on Epigenetic
% Robotics, Providence, USA, 08/2015.
% check page numbers


%% This proposal has
%% many interesting properties

%% This process is claimed to effectively
%% minimize free energy in the brain. Free energy could be thought 
%% of as the brain's effort needed to support concurrent hypotheses in
%% order to predict (explain) the current sensory state.


%%  given by the
%% closeness of 
%% of  spike-time
%% dependent plasticity (STDP) involve . the basic relation in time of two
%% stimuli
%% In STDP this relation is
%% represented by . 

\subsection{Summary}
\myparb{Tappings summary}To summarize this section we highlight the
main features of tappings. They provide an information centric view on
developmental models. This view is independent of particular learning
algorithms, and it provides an upper bound \footnote{the joint entropy
  of all sensorimotor variables} on the amount of explanation a model
needs to accomplish. That bound is a reference for comparing different
models in terms of the fraction of maximum explanation. Tappings
facilitate the design of developmental models, algorithms and their
implementations by highlighting regularities in the design space and
being precise and explicit about time. Analysing two important model
types and their tappings shows to what extent different functional
roles are determined by the input / output relations, and the learning
algorithm respectively. These features all contribute to facilitate
systematic exploration of developmental models.


%% In Analysis of existing model variations lets us identify two principal
%% configurations that correspond with the functional roles that internal
%% models can have.
%in terms of information within their degrees of freedom.

%% an important point is that both types can use the
%% same learning algorithm and that different functions arise only from
%% the difference in the input / output assignments. 

%% , for example to answer questions about additional fundamental
%% internal model types
% \end{enumerate}

%%  Different models can be compared by looking at how they perform
%% at explaining a given set of observations.

%% \subsection{Example}

%% % should come earlier

%% % \begin{wrapfigure}{l}{0.6\textwidth}
%% \begin{figure}
%%   \centering
%%   % \begin{subfigure}[b]{0.45\textwidth}
%%     \includegraphics[width=0.45\textwidth]{img/p_tappings/tapping_example_pimped.pdf}
%%     \caption{Automatic door prediction example.}
%%     \label{fig:ex-automaticdoor}
%%   %\end{subfigure}
%% \end{figure}
%% % \end{wrapfigure}

%% \myparb{Example setting} 
%% %Let's look at an example we are hopefully all familiar with. 
%% The concept of Tappings will be explained in the following with a concrete example.
%% Consider an automated door with
%% %door opening robot, embedded in a building, and consisting of 
%% a motorized slide-door and an infrared range sensor mounted at the
%% top of the doorframe controlling the motors with thresholding and
%% refractory period. Everybody has experienced failure modes of such
%% doors for example by approaching from the side, being too small,
%% approaching too fast, etc. We want to improve door behaviour by using
%% a few sensor floor tiles in the area surrounding the door as shown in
%% \autoref{fig:ex-automaticdoor}. % \FIXMET{Use ``from the side'' case, more plausible?}.

%% % Next to tile \#3 there is a vending machine.

%% \myparb{Example step-through} We want to predict the activation of the
%% infrared sensor from the activations of the floor tiles. Essentially
%% this constitutes a conditioning task that predicts the
%% unconditioned stimulus (US) from the conditioned stimulus (CS). There
%% are two types of people in the lobby, those leaving the building and
%% those fetching refreshments. Obviously tile \#1 is a simple and
%% effective choice as an input to the predictor. Now we know the
%% tapping: the input is sensor tile \#1 activation at time $t-1$ marked
%% with a green circle and the target is infrared sensor activation at
%% time $t$, hardwired to the motors and marked with the red circle. This
%% arrangement combines temporal and intermodal association.

%% % Now how does the tapping look like? Figure?



%%  An obvious extension would be two additional sensor tiles
%% left / below of tile \#1 to capture approaches from the side.

% \footnote{We can almost make a legitimate case out of this example.}

%% \FIXMET{Introduce a real practical example here: system, learning
%%   task, temporal-modal spread.}

%% As an example, let us look at a robotic arm with one joint at the base
%% and one rigid link carrying the end-effector. Let's say that this
%% robot is mounted on the wall like a clock and can rotate freely any
%% number of times. A fixed controller sends a constant command to the
%% motor which reults in the arm going round in clockwise direction. Due
%% to the open-loop nature of the controller, the movement is slower in
%% the left half of the circle because of gravity.

%% The pure temporal prediction task would be to predict the next state
%% based on the current state. Since the current state contains the
%% information about wether the arm is on the left or right part of the
%% circle, the predictor will be able to predict two different mean
%% velocities.

%% An intermodal association example would be to learn a mapping from a
%% measurement of angle to a measurement of the cartesian position of the
%% end-effector.

%% This robot can reach points on
%% a circle around its base with radius link-length. Say we want an agent to learn to control an
%% arm with one joint. If the agent manages to successfully learn this
%% task, we will be able to tell it to move the end-effector to a
%% particular position on ee-circle and the agent will generate to
%% correct command based on the current state (where it is right now) and
%% actually move there up to some finite degree of precision.

%% Internally, we define the state as a cartesian position $x,y$ and
%% the command $m$ is an angular velocity defined on a 10-bit resolution
%% servo interface. The learning task then consists in finding $g$ such that

%% $$f(x,y,m) = x,y +  + f_1(m) = x_d,y_d = $$

%% and the inverse

%% $$i(x,y,x_d, y_d) = m$$

%% such that

%% $$f(x,y,m) = |x_d,y_d - n| < \epsilon$$

\section{Basic tappings}
\label{sec:org1df4029}

%% Before we can proceed we need to distinguish between
%% stateless models having no memory (maps, feedforward neural networks)
%% and stateful models which do have memory (systems, recurrent neural
%% networks). For the rest of the paper we only deal with stateless
%% models and restrict ourselves to discuss tappings and stateful models
%% in the outlook.

%% \FIXMET{unclear but
%%   important} It depends on what is inside the predictor box how much
%% of the state's past is effectively being tapped to compute the
%% predictions, that is, the memory capacity, denoted $M$, of the
%% predictor, see paragraph 27 %???  below. 


\myparb{Variations} In this section we explore tappings further by
looking at some variations of the simple ones that came out of the
previous section: multi step prediction, autoencoding, and
autopredictive encoding. \myparb{Simple predictor} If the internal
model is a feedforward map without internal memory the simple one time
step predictor in \autoref{fig:ex-tpg-simplepred} cannot make use of
additional information about the future that was presented more than
one time step ago. The missing memory
of the model can be replaced by using a \emph{moving window} of
size $k$ that augments the momentary model input by including all $k$
previous values of the variables \footnote{The moving window technique
  is alternatively known as moving average model, time delay neural network,
delay-embedding or method of delays}. Since tappings are moving
windows, the multi time step tapping shown in
\autoref{fig:ex-tpg-multipred} is almost trivial, the window size
being equal to the number of input taps spread uniformly into the
past. The interesting bit is that iterative predictions in extended
forward simulations demands better model accuracy. A reasonable
shortcut towards more accuracy is to improve the prediction with
imposing a long-term consistency constraint by extending the target
tapping into the future (using buffering in closed-loop learning).

% If an agent cannot afford the
% update delay in closed-loop bootstrapping the model needs to be
% learned offline in a consolidation step.

%% increase with the length of the multi step prediction
%% horizon and decrease with length of the input and target parts of the
%% tapping.

%% predicts at time \(t-1\) a variable's
%% state at time \(t\) based on the state at \(t-1\). At time \(t\) the
%% prediction can be corrected by an adaptation step. 

%% Readers familiar with signal processing
%% will also recognize the similarity to finite impulse response
%% filters. Obviously the same can be done on the modality axis.

%% Such a tapping closely resembles a
%% finite impulse response linear filter structure of $M$-th
%% order. Common filters can have a strong (and reasonable) contiguity
%neighbourhood? topology?  prior.
%% delayed copies of $M$ on the past
%% to select the inputs to a memoryless feedforward map.

% \begin{wrapfigure}{l}{0.6\textwidth}
\begin{figure}
  \centering
  % \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=0.45\textwidth]{img/p_tappings/ex_tpg_multipred_symmetric.pdf}
    \caption{The multi step predictor using a window on $k$ past values as
      instantaneuous input and, in the fully symmetric case a window
      on $k-1$ addtional future values as the target. The time
      indexing has been omitted for that case for less clutter.}
    \label{fig:ex-tpg-multipred}
  %\end{subfigure}
\end{figure}
% \end{wrapfigure}

%% A finite impulse response filter is a
%%       well-known example, with the filter's order determined by the
%%       window size. \FIXMET{Need to add symmetric extension into the future (RL multistep/eligibility}}

%%  conn reconstructs its input on the 
%% output side involving only one variable at one time \(t\).

%% get the same element-wise tapping which just tells us that information
%% is potentially distributed from any channel to any other channel.

%%  with a temporal relation, reflected in the distribution of input and target
%% tapping over two different time steps.

%% , is to distribute the input and target assignment over two timesteps.

%% The
%% internal representation should then not only statically code the input
%% in compressed space but also the dynamics.

%% bib clean: IMM2012-06284, lara2007prediction, nyamapfene06:_unsup_multim_neural_networ

\myparb{Autoencoder} A special case of a predictor is the
autoencoder. Its tapping is shown on the left in
\autoref{fig:ex-tpg-ae-ape}. Its target output is the same as its
input. In terms of the $\bm{XY}$ formulation with $\bm{X} = \bm{Y}$,
the autoencoder could only consist of wires. The added value of an
autoencoder comes exclusively from constraints on the intermediate
representation. Like prediction learning, autoencoding is an
unsupervised learning technique built with supervised learning. For
many unsupervised learning tasks. If we look at the tapping we see
that the information of each single variable on the input is
distributed to all other variables on the
output. \myparb{Auto-Predictive-Encoder} By a simple change of the
tapping we easily obtain an autopredictive encoder (APE) as the result
of pulling the autoencoder's input and output taps one time step
apart. The autopredictive encoder is not an established term but
multiple proposals for such architectures have in fact been made
\cite{NIPS2014_5549,DBLP:journals/corr/PatrauceanHC15,copete16:_motor}.
Applying the prediction constraint on the model has been shown to
increase the task-independence of latent space representations by
(Lotter et al. 2015, \cite{DBLP:journals/corr/LotterKC15}). In
the tapping we see immediatly that the prediction constraint 
encourages the model to represent the rules of change in the hidden
space. The APE tapping is shown in
\autoref{fig:ex-tpg-ae-ape}. \myparb{Multimodal encodings and
  conditional inference} With a simple variation of the APE tapping we
can implement another powerful constraint for latent space
representation without changing the model. One possibility is to
augment the training set by appending multiple copies of itself to the
original. Before appending it, a fixed proportion of randomly chosen
input entries in the copy is set to an inactive state. If taps are
allowed to be blocking the tapped data, the same can be achieved by
making a set of random tapping nodes to be blocking for every episode
of training data that is presented. This is sketched in
\autoref{fig:ex-tpg-mape}. This is a
version of the dropout regularization technique applied to the
dataset. Like the prediction constraint this results
in models that generalize better for incomplete inputs which is known
as conditional inference in the Bayesian view \cite{5604275,ngiam2011multimodal,NIPS2014_5279}.


%% It is straightforward to make this even more
%% general by considering multimodal input, which is of great interest to
%% robotics. In these settings the network is trained to find shared
%% representations for inputs from different modalities that correspond
%% to the same situation. A common technique is to randomly ``dropout''
%% elements or blocks of elements when presenting a datapoint to the
%% learner, for example by setting these elements to a special
%% ``no-input'' value, indicated with gray tapmarks in
%% \autoref{fig:ex-tpg-mape}. This enables the network to predict one or
%% more modalities from potentially incomplete input. In a Bayesian
%% context, this is known as conditional inference and captures
%% sensorimotor learning problems in full generality
%% \cite{nyamapfene06:_unsup_multim_neural_networ,lara2007prediction,5604275,ngiam2011multimodal,NIPS2014_5279}.
%% % \FIXMET{Make diagram for multimodal encoders and conditional inference}

\begin{figure}
  \centering
  % \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=0.35\textwidth]{img/p_tappings/tapping_multimodal_codec_family.pdf}
    \caption{Autoencoder (left) and autopredictive encoder
      (right). The AE's tapping is special because input and target
      coincide. Pulling the input and source apart over one timestep
      difference produces the autopredictive encoder. The prediction
      prior imposes additional structure on the hidden representation.}
    \label{fig:ex-tpg-ae-ape}
  %\end{subfigure}
\end{figure}

\begin{figure}
  \centering
  % \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=0.35\textwidth]{img/p_tappings/tapping_multimodal_codec_family_dropout_sep.pdf}
    \caption{This illustrates the input / output dropout technique
      applied to an autopredictive encoder that integrates inputs from
      two modalities. The technique can be implemented either by
      augmenting the training data or by using time variant tappings
      with a blocking control. Going through the diagrams from left to
      right they each represent a dropout configuration for one episode
      for starting with a complete tapping on the left, followed by input dropout,
      input and target dropout, and a random configuration.}
    \label{fig:ex-tpg-mape}
  %\end{subfigure}
\end{figure}

%% Knocking out portions of the input or target vector with
%%       ``ignore'' values can also lead to better hidden
%%       representations and can enable the AE to perform dynamic
%%       conditional inference tasks. The left-most group is an AE
%%       combining an exteroceptive and a proprioceptive modality. Over
%%       time the tapping is modulated to implement the knockout,
%%       indicated by the examples progressing to the right. This is an
%%       example for a dynamic tapping which consists of sampling from
%%       the combinations of input-target pairs.

% \FIXMET{figure scheduled for kill} 

%% \FIXMET{,multimodal stuff:
%%   Rongali (PAE), H. Lee
%%   https://papers.nips.cc/paper/5279-improved-multimodal-deep-learning-with-variation-of-information,
%%   quadrotor deep learning, place invariant deep learning
%%   arxiv:1505.07428v1 ...}


% \FIXMET{Check refs for autopredictive coder.}


% Variations of temporal/modal cross prediction / inference: Copete
% Nagai Asada

%% \begin{figure*}% [htb!]
%%   \centering
%%   \begin{subfigure}[b]{0.6\textwidth}
%%     \centering
%%     \includegraphics[width=0.8\textwidth]{img/p_tappings/ex_tpg_ae.pdf}
%%     \caption{Autoencoder}
%%     \label{fig:ex-tpg-ae}
%%   \end{subfigure}
%% %  \quad
%%   \begin{subfigure}[b]{0.3\textwidth}
%%     \centering
%%     \includegraphics[width=0.45\textwidth]{img/p_tappings/ex_tpg_ape.pdf}
%%     \caption{Autopredictive encoder}
%%     \label{fig:ex-tpg-ape}
%%   \end{subfigure}
%%   \caption{\label{fig:ex-tpg-ae-ape}Standard and predictive autoencoding.}
%% \end{figure*}


% \label{p:rnn}
%  \myparb{Predictors and autoregressive models}

\section{Application areas}
% \section{Tappings for common models}
\label{sec:tap-common}
% \subsection{Application areas}
%% Our introductory robot learning
%% example made use of the

% approach that is very common in

%% bib clean: Haruno98, Haruno:2001:MMS:1121128.1121130

\myparb{Developmental robotics} Internal modelling
\cite{craik43:_natur_explan} is an important concept used in
developmental robotics
\cite{Wolpert98,Demiris2006361,10.3389/frobt.2016.00039}.  An
underlying driving hypothesis is that predictive models enable
\emph{anticipatory} behaviour \cite{rosen12:anticipatory_systems}
which is more powerful than purely reactive behaviour. From the
developmental perspective this implies that some functions of a
developmental model must be provided by adaptive models of the
sensorimotor dynamics. Two basic functional types of internal models,
forward and inverse ones, have already been introduced as examples in
\autoref{fig:basic-idea} and are shown again as a pair of tappings in
\autoref{fig:ex-tpg-mdl-pair}. This highlights the rearrangement of
the direction of prediction without a change of
variables. Exploitation of adaptive models has also been described
above indicating different ways of predicting and evaluating future
options with forward models, or directly infering actions with inverse
models.

%% The applicability of
%% tappings for design and analysis of internal modelling architectures
%% should be evident from the preceding parts of the paper.



\begin{figure}% [htb!]
  % \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{img/p_tappings/ex_tpg_model_fwd.pdf}
    \caption{Forward}
    \label{fig:ex-tpg-mdl-fwd}
  \end{subfigure}
  \quad
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{img/p_tappings/ex_tpg_model_inv.pdf}
    \caption{Inverse}
    \label{fig:ex-tpg-mdl-inv}
  \end{subfigure}
  \caption{Tapping a single time step forward- and inverse model
    pair. The model's functions are determined by different relations
    over the same set of variables.}
    \label{fig:ex-tpg-mdl-pair}
\end{figure}


% This works because the models 

%% For these two types there is a fixed assignment of the model
%% input and output ports to  Such models are trained with prediction learning.
%% % \FIXMET{Craik, Rosen, Wolpert, Demiris, Adapt}

%% Well known temporal difference algorithms
%% are Q-Learning, SARSA, and Actor-Critic methods
%% \cite{Sutton98,Watkins1992,rummery:cuedtr94}.

%% bib clean: \cite{Sutton98,Watkins1992,rummery:cuedtr94}.


\myparb{Reinforcement learning} A popular method in reinforcement
learning is temporal difference learning. Temporal difference learning
is a family of algorithms to approximate a prediction target with a
recurrent estimate. The usual target is a \emph{value function} which maps
actions to a value. The estimate is bootstrapped by minimizing the
moment-to-moment value prediction error, which is ultimately grounded
in a primary reward signal. There exists
extensive theory in RL that deals with the problem of integrating
task-relevant information that is spread out in time, with two
fundamental concepts being involved. The first one
is that of \emph{multistep methods} which take care of consequences escaping
into the future. The second one are \emph{eligibility traces} which
capture causes vanishing into the past. Taken together they solve the
general delayed reward problem. Depending on the parameters a
corresponding tapping will be similar to the multi step predictor.

The importance of features and modalities and the information
contained in their mutual relations is less developed. The concepts
used in reinforcement learning can easily be remapped to internal
modelling terms and vice versa, making tappings immediatly applicable
to temporal difference learning problems. Looking at three basic
temporal difference learning algorithms, TD(0), Q-Learning and SARSA,
we see that they all approximate a target by updating from a one time
step difference. TD(0)'s target is a state value function $v$ while
for Q-learning and SARSA it is a state-action value function $q$
\cite{Sutton98}. The update rules all follow the same general form of

\[
\Delta v = \alpha (R_t + \gamma v(S')_t)
\]

and the corresponding tappings are shown in
\autoref{fig:ex-tpg-rl-td}. Comparing these with the internal model
tappings we see that temporal difference learning corresponds with
prediction learning and that the value function is a forward model
allowing us to reframe a RL problems as developmental prediction
learning ones and the other way round.

%% % taken from RL_Slides_20170110.org

%% \[\begin{array}{rcl}
%% V(S) & \leftarrow & V(S) + \alpha \left(R + \gamma V(S') - V(S)\right) \\% _{ABt} \\
%% \end{array}\]

%% which translates to 

%% \[
%% V_(S)_{t+1} = (1 - \alpha) V(S)_t + \alpha (R_t + \gamma V(S')_t)
%% \]

%% which is equal to a Bayes filter update rule.

%% In the picture we have
%% extended the use of the target color ({\color{green}green}) to
%% indicate the variables taking part in computing the targets $v$ and
%% $q$ respectively.

%% \begin{figure*}% [htb!]
%%   \centering
%%   \begin{subfigure}[b]{0.3\textwidth}
%%     \centering
%%     \includegraphics[width=0.42\textwidth]{img/p_tappings/ex_tpg_bayes_filter_v2.pdf}
%%     \caption{Bayes filter.}
%%     \label{fig:ex-tpg-bayes-filter}
%%   \end{subfigure}
%%   \quad
%%   \begin{subfigure}[b]{0.6\textwidth}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{img/p_tappings/ex_tpg_rl_td_v3.pdf}
    \caption{Tapping temporal difference learning algorithms.}
    \label{fig:ex-tpg-rl-td}
\end{figure}
%%   \end{subfigure}
%%   \caption{Here we introduce additional computation edges drawn in
%%     gray to indicate the arguments for computing the target. a) Bayes
%%     filter: we use $u$ at $t-1$ because we want to use the latest
%%     state estimate to compute the new action. target x itself is
%%     computed recursively inside the filter. This is similar to b)
%%     TD(0) reinforcement learning variants, which recursively compute a
%%     target $v$ or $q$ from a measurement and a prediction.}
%% \end{figure*}

%% \FIXMET{facts:
%%  multistep bootstrapping, elgibility, tyranny of the time step,
%%  Methods in which the temporal difference extends over n steps are
%%  called n-step TD methods.}

% \FIXMET{refs: Actor-Critic, discuss Policy gradient}.

% \begin{figure}
\begin{wrapfigure}{l}{0.2\textwidth}% [htb!]
    \centering
    \includegraphics[width=0.19\textwidth]{img/p_tappings/ex_tpg_conditioning.pdf}
    \caption{Classical conditioning model requiring prediction of the
      unconditioned stimulus from another stimulus preceding the
      unconditioned one by a few time steps.}
    \label{fig:ex-tpg-conditioning}
\end{wrapfigure}
%\end{figure}

% bib clean: dayan16:_theor_neuros

\myparb{Neuroscience} Models of classical conditioning in neuroscience,
like the Rescorla-Wagner rule \cite{rescorla72:_pavlov}
provide links between the computational and neurobiological accounts
of reinforcement learning. Such models describe how an association is
learned across two modalities, the unconditioned (US) and the
conditioned stimulus (CS), and across two time steps, the CS preceding
the US. At the level of functional
organisation the reward prediction error hypothesis of dopamine
\cite{Schultz1593,Dayan02,Niv2009139}, and more recently, the
predictive-brain hypothesis \cite{e14112100,Clark.2015} carry
predictive coding ideas to the extreme. The claims are that the
information flow in the brain consists of top-down predictions and
bottom-up prediction errors, and that the brain is organised in
adaptive layers that learn to predict signals ascending from lower
layers with the help of predictions descending from higher
layers. Only the prediction error is being passed on to higher layers
which thereby becomes the main drive of activity. Tappings can again
be applied at all of these different levels of investigation.


%% More recent low-level descriptions of neural adaptation
%% use a characteristic asymmetric window. Stimuli are represented with
%% time intervals measured between to neural spikes. The window
%% is part of the rule for updating a directed
%% associative link between two neurons. The update strength is inversely
%% proportional to the inter-spike interval with potentiating direction
%% for causal sequences and a inhibting direction for acausal ones. This
%% process involves microscopic timescales but the fundamental issue of
%% associating points in the space of time and modality (SMT) remains
%% unchanged \cite{gerstner96,Markram213}.


%list models

%% Let's now look at tappings for some algorithms commonly used in
%% robotics to enable adaptive behaviour. \FIXMET{important?}

%% \myparb{Forward model}
%% Variables wired to motor units (actions) have special significance in
%% model learning. By adding an action to the inputs of a simple
%% predictor, it becomes a forward model, shown in
%% \autoref{fig:ex-tpg-mdl-fwd}. That means, the prediction for the state
%% at \(t+1\) is not only based on the current state but also on an
%% action. The action is assumed to be causally connected with the state
%% dynamics. Empirically this will be reflected in consistent
%% interactions of the action with the change in observed
%% variables. Independent of the interpretation it will improve the
%% predictability of the future state target. \myparb{Inverse model} An
%% inverse model in turn consumes the same variables as the forward model
%% but shuffles around the input and target assignments. The action
%% becomes the model's target representing the consistent contribution to
%% taking s\(_{\text{t}}\) to s\(_{\text{t+1}}\). Issues of invertibility
%% have to be dealt with by using %???
%% an appropriate learning machine, for
%% example probabilistic generative ones. An inverse model tapping is
%% shown in \autoref{fig:ex-tpg-mdl-inv}. Both models taken together form
%% a forward-inverse model pair.

% \FIXMET{fwd/inv example}

%% \FIXMET{bayes in/out, feels like a draft}
%% A tapping for another frequently used structure, the Bayes filter (BF), is
%% given in \autoref{fig:ex-tpg-bayes-filter} using naming conventions
%% from \cite[p. 24]{thrun00:_probab_robot}. Internally, a standard Bayes
%% filter has a predefined component containing a forward model,
%% computing a prediction $\hat{x}_{t-1}$ about the state $x_{t}$ from
%% $x_{t-1}$ and $u_{t-1}$. The BF is not usually updating that model,
%% but instead corrects the state input to the forward
%% model for the next iteration. The state itself is not directly
%% observable but is an inferred quantity, the only piece of new
%% information is the measurement $z$. This means the target needs to be
%% computed by an explicit rule from the primary variables, in the
%% simplest case as $x_t = \text{fwd}(x_{t-1}) + K (z_t - \text{fwd}(x_{t-1}))$ or
%% in probabilistic form as $p(x_t) = \eta p(z_t| x_t) \text{fwd}(x_{t-1})$. There are several interesting
%% perspectives on how to bootstrap the forward model as an
%% autopredictive encoder with multimodal input / target
%% pairs. Multimodality can be exploited as a regularizer with input /
%% target dropout in addition to the predictability prior for the
%% measurements. The hidden state $x$ from the BF now corresponds to the
%% APEs hidden layer activations which is already captured by the diagram
%% in \autoref{fig:ex-tpg-mape}. %\FIXMET{Make diagram for this scenario}.

%% under constraints
%% such as  prediction
%% constraints. 

%% including measurement
%% prediction.

%% and inferring the unobserved target with a maximum
%% Likelihood loss and regularization with predictability or incompleteness (input dropout) in a multimodal
%% case.

%  association under  and .
% a different model altogether.
% so there is an alternative tapping \autoref{fig:ex-tpg-bayes-filter-z}
% by
% with measurements weighted by their recurrently estimated statistics.

%% Feeding a
%% predictor's output back to its own input it can be 
%% turned into a generative model of the autoregressive (AR) family. This
%% feedback introduces memory via a global recurrence in the network and
%% is ideally suited for prediction learning using teacher forcing
%% \cite{williams89:_learn_algor_contin_runnin_fully}. The aim of
%% training is to be able to feed back the prediction to the input to
%% perform multistep sampling or self-sustained generation of a
%% timeseries that matches the original input statistics. AR models
%% have the same tapping as the simple predictor.


\section{Discussion}
\label{sec:discussion}

During our presentation of tappings a few issues have come up but
whose discussion was delayed for reasons of
simplicity. \myparb{Recurrence and autoregression} Models with memory
like recurrent neural networks need special consideration with respect
to tappings. Recurrent systems naturally retain an internal memory of
past input values. Such models do not need explicit memory in their
inputs and in theory only need to tap across one time step. They are
building up an implicit tapping as part of their learning. Measuring
the information flow across the model inputs and outputs after
training with quantitative \cite{Lungarella2005} or relational
techniques \cite{2010arXiv1004.2515W} should result in what could be
called effective tapping and this should be applicable to training
memoryless models.

%% This can be done information
%% theoretic methods  and  such
%% as partial information decomposition .

%% \myparb{Model basics} Want to learn correspondences (multifunctions), not
%% functions. Inference (probabilistic output and state repr), system
%% (recurrent, memory, time-variant), map (feedforward, memoryless,
%% time-invariant).

%% \myparb{Modelling baseline} Baseline is to just search the data anew
%% for every prediction.

%% \myparb{PI and the future} Not explicitly covered in the paper but it
%% is clear that the there are cases in which even the target needs to be
%% spread out over time and not come from only a sinlge time step. Goes
%% into multipre

\myparb{Info loss} The memory issue is an example of a more general
aspect about tappings. In the current state of our proposal, tappings
disregard details about the learning algorithm used at the level of
sensorimotor models. The same is evident in the case of inverse
problems where we needed to consider learning of correspondences
instead of functions. It remains to be shown how these properties
could be represented in a tapping.

%% The 
%% current state of our propposal tapping we have to demand that these issues are taken care of
%% separately to make sure that an algorithm is uesd which is actually
%% capable of representing the relations provided.

%% The upside is that 
%% algorithms with these properties do exist and we are only missing a
%% way of fully representing the issue in tappings.

%% The information which we
%% lose about the functional interaction is recovered by the function
%% approximation skills of adaptive sensorimotor models?
%% \FIXMET{triangular diagram}.

%% \myparb{Manifold} For completeness mention the manifold.

%% One challenge for scaling up tappings to large
%% spaces are sparse patterns with large spatial extent which could be
%% solved with graphical methods.

\myparb{Open issues} A final interesting issue is the problem of
changes in the tapping or the sensorimotor space itself that might
occur during a learning episode. When sketching the dropout constraint
for the autopredictive encoder a new tapping was drawn randomly for
each episode, which is a simple case of variation in time. We think it
is striaghtforward to obtain a more general time dependent formulation
of tappings. The tapping parameters could even be added to
sensorimotor space itself as interoceptive variables. Any advanced
developmental model will include an aspect of growth, just because in
open ended scenarios, it is not clear a priori how much explanatory
capacity is needed for a given level of accuracy in behaviour. If a
learning algorithm changes its own model size during learning, new
sensorimotor variables are either created or destroyed. If remains to
be seen if tappings can be extended to such cases in a meaningful way.


%% An ad hoc
%% solution 

%% would be to include some kind of dependency information in
%% the model with a mechanism attached for reacting to changes in
%% sensorimotor space. 



%% the.
%% dynamic tappings
%% that change during a learning episode. In a fixed sensorimotor space
%% only the tapping can change but with interceptive variables we also
%% need to consider adding rows to the sensorimotor trajectory matrix and
%% extend any tapping.

%% asking for
%% general graphical methods like grouping and hierarchical composition, which are available
%% \FIXMET{expand that}.

\section{Conclusion}
\label{sec:org91c9ccc}

%%  The embodiment creates the sensorimotor data on which  and the relations that 
%% systematic discussion of an important transformation step that is present in many

%% developmental models from various fields.  sensorimotor 
%% Tappings, a technique for designing and analyzing the integration of
%% supervised learning modules in larger models of agent development and
%% adaptive behaviour.

\myparb{Summary} We have presented tappings, a novel concept for
designing and analysing models of developmental learning in the field
of developmental robotics and the related fields of reinforcement learning and computational
neuroscience. Tappings came out of a need for capturing the detailed
embedding of learning machines in the temporal and modal context of
raw sensorimotor trajectories. Tappings create a particular view on
the interaction between the embodiment and the functional requirements
of behaviour that can help to better understand 
developmental learning processes, and make sensorimotor learning more efficient. They can systematically describe the
relationship between supervised learning and developmental models. By
ignoring computational details the tapping view highlights the
information flow across models and using that we can compare a large
range of models that cannot easily be compared otherwise. We showed
the structural similarity of prediction learning in the developmental
context and temporal difference learning in RL. Using tapping
manipulations we arrived at a learning scheme based on a predictive
version of the autoencoder which we think is a candidate for a general
building block in developmental models.

%% but which could 
%% benefit comparison. The
%% information flow can be made quantitative using information theoretic
%% measures. 

%% can be applied before, during, and
%% after learning to guide the selection of sensorimotor variables,
%% design of objectives and analysis of model performance.

%% , regardless of their
%% philosophical origin. %They highlight the  ??


% \FIXMET{De-capitalize Tappings, Neuroscience, ...}




%% large number of
%% variables. It is a rough sketch of the concept
%% and it needs to be explored further. There are notational issues such
%% as clarifying the notation about \emph{prediction} time and
%% \emph{predicted} time, distinguishing overall computation
%% \emph{models} and subordinate adaptive \emph{models}. How to deal with
%% dynamic creation and removal of interoceptive variables? For very
%% large tapping patterns, for example created using RNNs or interleaved
%% convolution, some symbols for common connection patterns need to be
%% explored. \FIXMET{Large-scale patterns of tappings, hierarchical relations,
%% procedural tappings, features on tappings.}


